Data-Driven Distributionally Robust System Level Synthesis

We present a novel approach for the control of uncertain, linear time-invariant systems, which are perturbed by potentially unbounded, additive disturbances. We propose a \emph{doubly robust} data-driven state-feedback controller to ensure reliable performance against both model mismatch and disturbance distribution uncertainty. Our controller, which leverages the System Level Synthesis parameterization, is designed as the solution to a distributionally robust finite-horizon optimal control problem. The goal is to minimize a cost function while satisfying constraints against the worst-case realization of the uncertainty, which is quantified using distributional ambiguity sets. The latter are defined as balls in the Wasserstein metric centered on the predictive empirical distribution computed from a set of collected trajectory data. By harnessing techniques from robust control and distributionally robust optimization, we characterize the distributional shift between the predictive and the actual closed-loop distributions, and highlight its dependency on the model mismatch and the uncertainty about the disturbance distribution. We also provide bounds on the number of samples required to achieve a desired confidence level and propose a tractable approximate formulation for the doubly robust data-driven controller. To demonstrate the effectiveness of our approach, we present a numerical example showcasing the performance of the proposed algorithm.

==> sections/formulation.tex <==
\twocolumn
\section{Problem formulation}\label{Sec:Problem_Formulation}
Consider a discrete-time linear time-invariant (LTI) system
\begin{equation*}\label{eq:Dynamics}
    x_{k+1}={A} x_{k} + {B} u_{k} +\xi_{k}\ ,
\end{equation*}
with (fully measurable) state $x_k \in \mathbb{R}^{n}$, control input $u_k \in \mathbb{R}^{m}$. The system is affected by the additive disturbance $\xi_k \in \mathbb{R}^{n}$ distributed according to some unknown probability distribution $\mathbb{P}_{\xi}$ defined over the unknown and possibly unbounded support set ${\Xi} \subseteq \mathbb{R}^{n}$. 

In this paper, we are interested in a finite horizon control problem of horizon length $T$. Let us introduce the following $T$-step matrix formulation of the dynamics
\begin{equation}\label{eq:dynamics_matrix_form}
    \bs{x}=L \bs{z} + \bs{w},
\end{equation}
where we concatenate the states, inputs, and noises of the system into stacked vectors
\begin{equation*}
\bs{x}=\!\begin{bmatrix}
        x_{1} \\
        x_{2} \\
        \vdots \\
        x_{T}
    \end{bmatrix}, \ \bs{u}=\!\begin{bmatrix}
        u_{0} \\
        u_{1} \\
        \vdots \\
        u_{T\!-\!1}
    \end{bmatrix}, \ \bs{\xi}=\!\begin{bmatrix}
        \xi_{0} \\
        \xi_{1} \\
        \vdots \\
        \xi_{T\!-\!1}
    \end{bmatrix}, \ \bs{z} =\! \begin{bmatrix}	x_0 \\ \bs{u} \end{bmatrix},\ {\bs{w}} =\! {H} \bs{\xi},
\end{equation*}

\begin{align*}%\scalemath{0.8}{
        {{L}}&=
        \begin{bmatrix}
            {A} & {B} & 0_{n\! \times\! m} & \cdots & 0_{n\! \times\! m} \\
            {A}^{2} & {A} {B} & {B} & \ddots & \vdots \\
            \vdots & \vdots & \ddots & \ddots & 0_{n\! \times\! m} \\
            {A}^{T} & {A}^{T-1} {B} & \cdots & {A} {B} & {B}
        \end{bmatrix},\, %}\end{equation*}
%		\begin{equation*}\scalemath{0.82}{ 
\\
    {{H}}&=
        \begin{bmatrix}
            I_{n\! \times\! n} & 0_{n\! \times\! n} & \cdots & 0_{n\! \times\! n} \\
            {A} & I_{n\! \times\! n} & \ddots & \vdots \\
            \vdots & \ddots & \ddots & 0_{n\! \times\! n} \\
            {A}^{T-1} & \cdots & {A} & I_{n\! \times\! n}
        \end{bmatrix}.
\end{align*}
For notational compactness, we introduce $\bs{z}$ to include both the initial condition $x_0$ and the control input sequence $\bs{u}$. The multi-step disturbance ${\bs{w}} \in \mathcal{W} \subseteq \mathbb{R}^{nT}$ distributed according to $\mathbb{P}_{\bs{w}}$. 

Our objective is to design an optimal control policy which minimizes a cost function while satisfying constraints over a finite horizon $T$. Formally, a policy $\pi=\{\pi_{t}(\cdot)\}_{t=0}^{T-1}$ is a collection of causal and measurable functions, where each function $\pi_t:\mathbb{R}^{(t\!+\!1)n}\rightarrow \mathbb{R}^m$ maps past states to the next control action, that is $u_t=\pi_t(x_0,\dots,x_t)$.

Define $\bs{y} := \begin{bmatrix} \bs{z}^\top&\bs{x}^\top\end{bmatrix}^\top\in\mathbb{R}^{n+T(m+n)}$ and denote with $\Pcl$ the closed-loop distribution of $\bs{y}$ induced by the model $L$ under the policy $\pi$ . (We will keep $H$ unknown but constant throughout the paper.) Now, we can formulate the following finite horizon stochastic optimal control problem

\begin{equation}\label{eq:MPC_problem_y}
    \begin{aligned}
        {J} := \min_{\pi} \quad & \mathbb{E}^{\bs{y}\sim \Pcl} \left[ h\left(\bs{y}\right) \right]\\
        \text{s.t.}	\quad & \text{CVaR}_{1-\beta}^{\bs{y}\sim \Pcl} \left[g(\bs{y})\right] \leq 0 \\
    \end{aligned}\ ,
\end{equation}
where $h:\mathbb{R}^{n+T(m+n)}\rightarrow \mathbb{R}^+$ is the objective function, and $g:\mathbb{R}^{n+T(m+n)}\rightarrow \mathbb{R}$ the constraint function.
Due to stochasticity, the cost is minimized in expectation and the constraint $g\left( \bs{y}\right)\leq 0$ 
on the future states and inputs is imposed as a Conditional Value-at-Risk (CVaR) constraint, which is defined below.
\begin{Definition}[Conditional Value-at-Risk]
    For a random variable $\omega\in\Omega\subseteq\mathbb{R}^r$ with distribution $\mathbb{P}_{\omega}$ and a function $\phi:\mathbb{R}^r\rightarrow\mathbb{R}$, the CVaR of level $\beta$ is defined as
    \begin{equation*}
        \text{CVaR}_{1-\beta}^{\omega\sim\mathbb{P}_{\omega}}\left(\phi(\omega)\right):= \inf_{t \in \mathbb{R}} \left[{\beta}^{-1}\, \mathbb{E}^{\omega\sim\mathbb{P}_{\omega}}\left[\left(\phi(\omega) +t\right)_{+}\right]-t\right]\ .
    \end{equation*}
\end{Definition}

To deal with the stochasticity of problem~\eqref{eq:MPC_problem_y} we assume that we are given trajectory data, generated by system~\eqref{eq:dynamics_matrix_form}.
\begin{Assumption}[Data Collection]\label{Ass:data}
We have access to trajectory data in the form of a dataset $\mathcal{D}^{N,T}$, comprising $N$ independent $T$-step input-state trajectories $\begin{bmatrix}
    \bs{z}^i \\ \bs{x}^i
\end{bmatrix}$, $i=1,\dots,N$, that have been collected by applying inputs $\bs{u}^i$ of length $T$ to system~\eqref{eq:dynamics_matrix_form}, starting from some initial condition $x_0^i$. The corresponding disturbance trajectories are denoted by $\bs{w}^i$.
\end{Assumption}

We also assume that the noise distribution and the system dynamics are uncertain, which makes solving~\eqref{eq:MPC_problem_y} more challenging. 
  \begin{Assumption}[Uncertain model]\label{Ass:Spectral_norm_bound}
  The noise distribution $\Prob_{\bsw}$ is unknown. The system model is uncertain. The true model $L$ lies within a $\gamma$ ball around a system estimate $\hat{L}$
    \begin{equation*}
      \opnorm{\Delta L} := \opnorm{L-\hat{L}} \leq \gamma,
    \end{equation*}
    for some $\gamma>0$ with $\opnorm{\cdot}$ the spectral norm. The estimate $\hat{L}$, and thus the model error $\opnorm{\Delta L}$ have the same lower triangular structure as $L$.
  \end{Assumption}
For clarity of exposition we are assuming here that this bound is provided and deterministic. In practice, the model estimate $\hat{L}$ can be the output of some identification procedure that exploits input-state T-steps trajectories collected from the system in a similar fashion as the dataset $\mathcal{D}^{N,T}$. The results in this in this paper can be easily extended to setting where this bound is in the form of a probabilistic bound, as common for stochastic estimation processes. 
\fm{See for example [add citations][][][].}

Even with perfect knowledge of the model, optimizing~\eqref{eq:MPC_problem_y} over general policies can be intractable due to the inherent challenge of dealing with an infinite-dimensional problem. Therefore, we will focus on the class of disturbance-affine causal feedback policies of the form 
    \begin{equation*}
v_t+\sum_{i=0}^{t-1}\Gamma_{t,i}w_{t-i-1},\,t=0,\dots,T-1,
\end{equation*}
parameterized by an open-loop input component $v_t$ and a sequence of feedback gains $\Gamma_{t,i}$, for $i=0,\dots,t-1$. 
Note that the feedback policy must be a function of the observables, e.g. the state sequence $\bs{x}$. We can compute the disturbance $\bs{w}$ only through the \emph{unknown} model $L$. Since we only have access to an approximate model $\hat{L}$, the above policy is not implementable. Instead, we can approximate the disturbances $\bsw$ by computing the \emph{certainty equivalent} differences $\hat{\bsw}=\bs{x}-\hat{L}\bs{z}$, leading to the class of parameterized policies
\begin{equation}\label{eq:affine_policy_wrong_model}
\pi_t(x_0,\dots,x_t)=v_t+\sum_{j=0}^{t-1}\Gamma_{t,i}\hat{w}_{t-j-1},\,t=0,\dots,T-1,
\end{equation}
 Under policy~\eqref{eq:affine_policy_wrong_model}, following the convention of~\eqref{eq:dynamics_matrix_form}, we can write
 $$\bs{u} = \bs{v}_u + \Gamma_u (\bs{x}-\hat{L}\bs{z}) \ ,$$
 where $\bs{v}_u:= \begin{bmatrix}v^\top_0&\dots&v^\top_{T-1} \end{bmatrix}^\top$ and 
 % $\Gamma_u \in \mathbb{R}^{Tm\times Tn}$  
	\begin{equation}\label{eq:AffinePolicy} \Gamma_u = 
	\begin{bmatrix} \bs{0}_{m\times n} &\bs{0}_{m\times n} & \dots &\bs{0}_{m\times n} & \bs{0}_{m\times n} \\
		 \Gamma_{1,0} & \bs{0}_{m\times n} &  & \bs{0}_{m\times n}& \bs{0}_{m\times n}\\
		  \Gamma_{2,0} & \Gamma_{2,1} & &  &  \\ 
		 \vdots & \vdots & \ddots &  &\vdots \\ 
		\Gamma_{T\minus1,0} & \Gamma_{T\minus1,1} & \dots & \Gamma_{T\minus1,T\minus2} & \bs{0}_{m\times n} \end{bmatrix}
	\end{equation}
is the lower triangular causal feedback matrix induced by the feedback gains. 
 The structure of $\Gamma_u$ is a consequence of the causality constraint that enforces the control input at time $t$ to depend on the history up to time $t$. To further reduce the notation overhead, we introduce
\begin{equation} \label{eq:AffinePolicy_extension}
\Gamma = 
    \begin{bmatrix} \bs{0}_{n\times Tn} \\
        \Gamma_u
    \end{bmatrix}, \quad 
    \bs{v} = \begin{bmatrix} x_0 \\
    \bs{v}_u
    \end{bmatrix}.
\end{equation}
With this new notation, we can write $\bs{z}=\bs{v}+\Gamma (\bs{x}-\hat{L}\bs{z})$, where the first block entry of $\bs{z}$ represents the initial condition.


Disturbance-affine policies have been shown to provide a good trade-off between tractability and performance, and have been widely used in the control systems literature \fm{add reference
[Optimization over state feedback policies for robust control with constraints]} to reduce the conservatism of open-loop policies. However, in the presence of uncertain dynamics and statistics, we have the additional challenge of robustness. Simply optimizing policies based on approximate system models and statistics might lead to poor closed-loop performance, as we review in Section~\ref{sec:SAA}. However, by designing distributionally robust controllers, we can systematically trade-off nominal performance and robustness, as explored in Section~\ref{Sec:DR_Formulation}.

\section{Sample Average Approximation approach}\label{sec:SAA}
Given trajectory samples and the approximate model $\hat{L}$, we can construct a ``certainty equivalent" empirical disturbance distribution  as follows 
$$\hat{\bs{w}}\sim \hat{\mathbb{P}}_{\hat{L}}^{\bs{w}} := \frac{1}{N} \sum_{i=1}^{N} \delta_{\hat{\bs{w}}^{i}}\ ,\ \text{ with }\ \hat{\bs{w}}^{i}= \bs{x}^i -\hat{L}\bs{z}^{i},$$
where $\hat{\bs{w}}^i$, $i=1,\dots,N$ are the residual errors between actual and predicted states.
The term ``certainty equivalent" refers to the fact that we trust, for the moment, the model $\hat{L}$ to be accurate.
In a similar fashion, we can compute empirical predictive distributions of inputs and states under the disturbance-affine feedback policy $\pi$ defined in~\eqref{eq:affine_policy_wrong_model}.
For the joint vector $\bs{y} := \begin{bmatrix} \bs{z}^\top&\bs{x}^\top\end{bmatrix}^\top$, we have 
\begin{equation}\label{eq:predictive_empirical_distribution}
\Pemp = \frac{1}{N} \sum_{i=1}^{N} \delta_{\hat{\bs{y}}^{i}},
\end{equation}
where the certainty equivalent predictions are
$$\hat{\bs{y}}^{i} := \begin{bmatrix}
        \bs{v} + \Gamma \hat{\bs{w}}^i \\ \hat{L}(\bs{v} + \Gamma \hat{\bs{w}}^i )+\hat{\bs{w}}^i
    \end{bmatrix}.$$
The meaning of the notation is as follows: $\bar{\Prob}$ symbolizes that we are dealing with empirical distributions and the subscript $\pi,\hat{L}$ implies that we are considering the distribution induced by the policy~\eqref{eq:affine_policy_wrong_model} and dynamics $\hat{L}$. 

A possible solution to problem~\eqref{eq:MPC_problem_y} is optimizing the empirical predicted performance, also known as Sample Average Approximation (SAA). 
\begin{equation}
\label{eq:MPC_problem_SAA}
 \begin{aligned}
            {J}_{\tau}^{SAA} := \min_{\bs{v},\Gamma} \quad & \mathbb{E}^{\bs{y}\sim \Pemp}[h(\bs{y})]\\
            \text{s.t.}	\quad & \text{CVaR}_{1-\beta}^{\bs{y}\sim \Pemp} \left(g(\bs{y})\right) \leq 0,~\eqref{eq:affine_policy_wrong_model},~\eqref{eq:AffinePolicy_extension}
        \end{aligned}
    \end{equation}
The expectations in the cost and in the constraint are taken with respect to the empirical predictive distribution $\Pemp$.  This can also be referred to as the \textit{in-sample} optimization problem in the optimization literature or as the Empirical Risk Minimization in the operation research literature. \fm{add references}. 

The SAA formulation has the advantage of being tractable and having strong asymptotic performance guarantees. However, if the model error $\hat{L}-L$  is significant and the number of samples $N$ is small, then the SAA approach might suffer from poor closed-loop performance. It can overfit to the wrong model $\hat{L}$ and the samples $\bs{z}^i,\,\bs{x}^i$, for $i\le N$, leading to optimistically biased solutions. This, in turn, can result in large \textbf{distribution shift} between the \textit{in-sample} distribution $\Pemp$ and the \textit{out-of-sample} distribution $\Pcl$. 
In the following section we adopt a distributionally robust formulation, compensating for this distribution shift, which is fundamental in data-driven control.
\tas{Would be nice to have a figure here where the DRO works while CE fails} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Distributionally robust formulation}\label{Sec:DR_Formulation}	
A fundamental limitation of Sample Average Approximation is the discrepancy between in-sample predicted performance and out-of-sample closed-loop performance. 
To account for this distribution shift, we follow a distributionally robust approach. We robustify problem~\eqref{eq:MPC_problem_SAA} against uncertainties in the predictive distributions, by optimizing over the worst-case expectation within a set of probability distributions, also known as an ambiguity set. 

In this paper, we consider ambiguity sets constructed using the Wasserstein metric, which provides a measure of dissimilarity between two probability distributions. The Wasserstein metric quantifies the minimum cost required to transform one distribution into another, with the cost being defined as the integral of the transportation cost across the probability distribution space.
\begin{Definition}[Wasserstein metric~\cite{kantorovich1958space,mohajerin2018data}]
    Consider distributions $\mathbb{Q}_1,\mathbb{Q}_2 \in \mathcal{M}(\mathcal{Y})$, where $\mathcal{M}(\mathcal{Y})$ is the set of all probability distributions $\mathbb{Q}$ supported on $\mathcal{Y}$ such that $\mathbb{E}^{\mathcal{Y}}\left[\| \bs{x} \|\right] < \infty $.
    The Wasserstein metric $d_{\mathrm{W}} : \mathcal{M}(\mathcal{Y}) \times \mathcal{M}(\mathcal{Y}) \rightarrow \mathbb{R}_{\geq 0}$ between the distributions $\mathbb{Q}_1$ and $\mathbb{Q}_2$ is defined as
    %
    \begin{equation}\label{eq:Wasserstein_distance}\scalemath{0.84}{
            d_{W}\!\left(\mathbb{Q}_{1}, \mathbb{Q}_{2}\right):=\inf_{\Pi} \left\{\int_{\mathcal{Y}^{2}}\left\|\bs{x}_{1}-\bs{x}_{2}\right\| \Pi\left(\mathrm{d} \bs{x}_{1}, \mathrm{d} \bs{x}_{2}\right)\right\},}
    \end{equation}
    where $\Pi$ is the joint distribution of $\bs{x}_1$ and $\bs{x}_2$ with marginals $\mathbb{Q}_1$ and $\mathbb{Q}_2$. \tas{define the norm}
\end{Definition}
\tas{goes elsewhere?} The Wasserstein metric is a popular choice for defining ambiguity sets as it can handle distributions with arbitrary supports, and it can be defined using a finite number of sample points, making it computationally tractable for data-driven applications.  Other types of ambiguity sets, such as those based on the Kullback-Leibler divergence or the total variation distance, may have disadvantages such as not being a true metric or not being defined for distributions with different supports. 
\td{expand on the cons of other types of ambiguity sets and add references.}\tas{not here maybe in intro}

We can now define a Wasserstein ambiguity set as the set of all probability distributions that are within a certain Wasserstein distance (Wasserstein radius) from some nominal distribution (here the empirical distribution).
An ambiguity set of radius $\varepsilon>0$ around a probability measure $\Prob$ is defined as:
\begin{equation}
\mathcal{B}^{\varepsilon}\left(\Prob\right) := \left\{\mathbb{Q}\in \mathcal{M}(\mathcal{Y})\middle| d_{W}\!\left(\Prob,\mathbb{Q}\right)\leq \varepsilon \right\}.
\end{equation}
	
The distributionally robust (DR) FHOC problem can now be written as
\begin{equation}\label{eq:DR_MPC_1}
    \begin{aligned}
            {J}^{DR} :=& \min_{\bs{v},\Gamma}  &&\sup_{\mathbb{Q} \in \mathcal{B}^{\varepsilon}\left(\Pemp\right)} \mathbb{E}^{\bs{y}\sim\mathbb{Q}}\left[ h\left(\bs{y}\right) \right]\\
            &\text{s.t.} \quad &&\sup_{\mathbb{Q} \in \mathcal{B}^{\varepsilon}\left(\Pemp\right)}\text{CVaR}_{1-\beta}^{\bs{y}\sim\mathbb{Q}}\left(g(\bs{y})\right) \leq 0, 
            % \quad & x_0 = x_{\tau} \\
            % \quad & \bs{z} = \pi(x_0, \bs{w}, A, B, \bs{v}, \Gamma) \ 
            \\
            & && \eqref{eq:affine_policy_wrong_model},~\eqref{eq:AffinePolicy_extension}
    \end{aligned}
\end{equation}

The ambiguity set $\mathcal{B}^{\varepsilon}\left( \Pemp\right)$ is a ball defined with respect to the Wasserstein metric~\eqref{eq:Wasserstein_distance}. The ball is centered around the empirical predictive distribution $\Pemp$ and has a radius of $\varepsilon$. Similarly to the approach in [ref cdc paper francesco], the ambiguity set is centered on a distribution that depends on the optimization variables of the problem, namely $\bs{v}$ and $\Gamma$. It is worth noting that, as is common in robust optimization, the cost and constraint worst-case are formulated independently, possibly introducing some degree of conservatism due to the optimization problem optimizing against two separate worst-case distributions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For some policy  feedback matrix $\Gamma$, if the radius $\varepsilon$ is large enough then the ambiguity set will contain the actual closed-loop distribution $\Pcl$; it is sufficient to have $d_{W}(\Pemp,\Pcl)\leq \varepsilon$. In this case, solving~\eqref{eq:DR_MPC_1} will provide a control policy which is robust against distribution shifts with respect to the in-sample empirical distribution, including the actual closed-loop behavior. In order to achieve this, we need to characterize the distribution shift $d_{W}(\hat{\Prob}^y_{\pi,\hat{L}},\Prob^y_{\pi,L})$, which is the subject of Section~\ref{Sec:Shift}. Informally, this will allow us to show that if the distributionally robust problem~\eqref{eq:DR_MPC_1} is feasible and its minimizer $(\bs{v}^{DR}, \Gamma^{DR})$ attains a cost $J^{DR}(\bs{v}^{DR}, \Gamma^{DR})$, then, with high confidence, the policy $\pi$ in~\eqref{eq:affine_policy_wrong_model} is a feasible solution for the original Problem~\eqref{eq:MPC_problem_y} and the resulting cost ${J}(\bs{v}^{DR}, \Gamma^{DR})$ is upper bounded by the computed $J^{DR}(\bs{v}^{DR}, \Gamma^{DR})$. \tas{we need to be consistent with notation}

Even if we have an accurate radius $\varepsilon$, we still need to solve~\eqref{eq:DR_MPC_1}. The main challenge is reformulating~\eqref{eq:DR_MPC_1} in a way that makes the solution tractable. The main difficulty is that the shape of the ambiguity sets (the radius $\varepsilon$) depends on the control policy parameters $v,\Gamma$ as well as the uncertainty $\hat{L}-L$. In Section~\ref{Sec:Reformulation}, we employ techniques inspired by small-gain theory to obtain such a reformulation.

\tas{add any required assumptions on cost and noise here?}
\fm{Should we try to make the formulation more general? type-p wasserstein distance and more general cost?}

\tas{moved this here but we need to write why we need this
We require a technical assumption on the distribution of the multi-step noise $\bs{w} = {H} \bs{\xi}$.
\begin{Assumption}[Light-tail assumption]\label{Ass:Light_Tail}
    For some constants $a>1$ and $b>0$
    %		\vspace{-2pt}
    \begin{equation*}
            \mathscr{E}_{a,b} = \mathbb{E}\left[e^{b \|{\bs{w}}\|^a}\right]< +\infty\ .
    \end{equation*}
\end{Assumption}
\vspace{-2pt}
This assumption is a condition on the decay rate of the tail of the probability distribution $\mathbb{P}_{w}$ and it is trivially satisfied when $w\sim\mathbb{P}_{w}$ is sub-Gaussian or when $\mathcal{W}$ is compact. Similarly, one could make this assumption directly on the tail of the probability distribution $\mathbb{P}_{\xi}$, which would then imply light-tail-ness of the distribution $\mathbb{P}_{w}$ (because of linear transformation) even though the bound will then also depend on the unknown Toeplitz matrix ${H}$. This is not restrictive, as the values of $a$ and $b$ are not required in practice.
} 
\fm{This assumption is required to obtain the final sample concentration bound of Lemma~\ref{Lemma:fournier}}

